Analysis and Counterexamples Regarding Yatsenko's Polynomial-Time Algorithm for Solving the Traveling Salesman Problem

Yatsenko gives a polynomial-time algorithm for solving the traveling salesman problem. We examine the correctness of the algorithm and its construction. We also comment on Yatsenko's evaluation of the algorithm.

==> urcsmacros.tex <==
%
% urcsmacros
%
% author: Lawrence A. Crowl
% last updated: 28 April 1990
%
% BibTeX
%
\newcommand{\BibTeX}{{B\kern-.0833em{\sc ib}\kern-.1667em%
T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX}}
%
% SLiTeX
%
\newcommand{\SliTeX}{{\rm S\kern-.06em{\sc l\kern-.035emi}\kern-.06em
T\kern -.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%
% UNIX
%
\newcommand{\UNIX}{{\sc Unix}}
%
% trademark
%
\newcommand{\trademark}{$^{\rm TM}$}
%
% singlespacing (for use in doublespaced documents)
%
\def\doublespacefactor#1#2{%
\newenvironment{singlespace}{\baselineskip #2\baselineskip}%
{\par \baselineskip #1\baselineskip}%
\par \baselineskip #1\baselineskip}
%
% various latin abbreviations
%
\def\adhoc{{\em ad hoc}}
\def\aposteriori{{\em a posteriori}}
\def\apriori{{\em a priori}}
\def\Cf{{\em Cf.}}
\def\cf{{\em cf.}}
\def\Eg{{\em E.g.}}
\def\eg{{\em e.g.}}
\def\etal{{\em et al.}}
\def\etc{{\em etc.}}
\def\Ibid{{\em Ibid.}}
\def\ibid{{\em ibid.}}
\def\Id{{\em Id.}}
\def\id{{\em id.}}
\def\Ie{{\em I.e.}}
\def\ie{{\em i.e.}}
\def\Loccit{{\em Loc.\ cit.}}
\def\loccit{{\em loc.\ cit.}}
\def\Opcit{{\em Op.\ cit.}}
\def\opcit{{\em op.\ cit.}}
\def\qv{{\em q.v.}}
\def\Qv{{\em Q.v.}}
\def\viz{{\em viz.}}
%
% andbreak  (for breaking author lists)
%
\def\andbreak{%% \begin{tabular}
\end{tabular}\\\begin{tabular}[t]{c}%% \end{tabular}
}
%
% titlequote
%
\def\titlequote#1{\hfill
\parbox{4in}{\begin{flushright}{\small\it #1}\end{flushright}}}
%
% weekdaystring
%
% Dump the day of the week in string form.
% This macro is only valid from 1901 A.D. through 2099 A.D.
%
\def\weekdaystring#1#2#3{{% extra brace saves enclosing register state
%
% days through the end of the year
% days := current year * 365
\count10=#3%
\multiply\count10 by 365%
% leap years := year / 4
\count11=#3%
\divide\count11 by 4%
% days := days + leap years
\advance\count10 by \count11
%
% find out if the current year is a leap year
% last leap year := leap years * 4
\count12=\count11%
\multiply\count12 by 4
% years since last leap year := current year - last leap year
\count13=#3%
\advance\count13 by -\count12%
% years since last leap year equals zero when current year is a leap year
%
% subtract off those days in this month and the following months
% days = days - following days [ is leap ] [ current month ]
\ifcase#2%
\or\ifcase\count13\advance\count10 by -366% leap January
\else\advance\count10 by -365% normal January
\fi%
\or\ifcase\count13\advance\count10 by -335% leap February
\else\advance\count10 by -334% normal February
\fi%
\or\advance\count10 by -306% March
\or\advance\count10 by -275% April
\or\advance\count10 by -245% May
\or\advance\count10 by -214% June
\or\advance\count10 by -184% July
\or\advance\count10 by -153% August
\or\advance\count10 by -122% September
\or\advance\count10 by -92% October
\or\advance\count10 by -61% November
\or\advance\count10 by -31% December
\fi%
%
% update days by day of month
% days := days + current day
\advance\count10 by #1%
%
% find weekday number
% offset for initial day of the week
\advance\count10 by 5
% last monday := (current day / 7) * 7
\count14=\count10%
\divide\count14 by 7%
\multiply\count14 by 7
% weekday number := current day - last monday
\count15=\count10%
\advance\count15 by -\count14
%
% now dump out appropriate string
\ifcase\count15 Monday\or Tuesday\or Wednesday%
\or Thursday\or Friday\or Saturday\or Sunday\fi%
}}
%
% monthstring
%
% Dump the month in string form.
%
\def\monthstring#1{\ifcase#1\or January\or February\or March\or April\or May%
\or June\or July\or August\or September\or October\or November\or December\fi}
%
% dateWDMY
%
% Redefine \today as "weekdaystring daynumber monthstring yearnumber" format.
%
\def\dateWDMY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\number\day\space\monthstring{\month}\space\number\year}}
%
% dateDMY
%
% Redefine \today as "daynumber monthstring yearnumber" format.
%
\def\dateDMY{\def\today{\number\day\space\monthstring{\month}%
\space\number\year}}
%
% dateWMDY
%
% Redefine \today as "weekdaystring monthstring daynumber, yearnumber" format.
%
\def\dateWMDY{\def\today{\weekdaystring{\day}{\month}{\year}\space%
\monthstring{\month}\space\number\day,\space\number\year}}
%
% dateMDY
%
% Redefine \today as "monthstring daynumber, yearnumber" format.
%
\def\dateMDY{\def\today{\monthstring{\month}\space\number\day,%
\space\number\year}}
%
% dateMY
%
% Redefine \today as "monthstring yearnumber" format.
%
\def\dateMY{\def\today{\monthstring{\month}\space\number\year}}
%
% dateY
%
% Redefine \today as "yearnumber" format.
%
\def\dateY{\def\today{\number\year}}

